DOCE: Finding the Sweet Spot for Execution-Based Code Generation

Recently, a diverse set of decoding and reranking procedures have been shown effective for LLM-based code generation. However, a comprehensive framework that links and experimentally compares these methods is missing. We address this by proposing Decoding Objectives for Code Execution, a comprehensive framework that includes candidate generation, $n$-best reranking, minimum Bayes risk (MBR) decoding, and self-debugging as the core components. We then study the contributions of these components through execution-based evaluation metrics. Our findings highlight the importance of execution-based methods and the difference gap between execution-based and execution-free methods. Furthermore, we assess the impact of filtering based on trial unit tests, a simple and effective strategy that has been often overlooked in prior works. We also propose self-debugging on multiple candidates, obtaining state-of-the-art performance on reranking for code generation. We expect our framework to provide a solid guideline for future research on code generation.

==> sections/reviewer_prompt.tex <==
\begin{figure*}[hbt!]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### code
```python
def count_ways(n):
  A = [0] * (n + 1)
  B = [0] * (n + 1)
  A[0] = 1
  A[1] = 0
  B[0] = 0
  B[1] = 1
  for i in range(2, n+1):
    A[i] = A[i - 2] + 2 * B[i - 1]
    B[i] = A[i - 1] + B[i - 2]
  return A[n]
```

Write the docstring for the above code.

### docstring
```python
"""
Write a function to find the number of ways to fill it with 2 x 1 dominoes for the given 3 x n board.
>>> count_ways(2)
3
"""
```
### task end ###

### task start ###
### code
```python
import re
def find_char_long(text):
  return (re.findall(r"\b\w{4,}\b", text))
```

Write the docstring for the above code.

### docstring
```python
"""
Write a function to find all words which are at least 4 characters long in a string by using regex.
>>> find_char_long('Please move back to stream')
['Please', 'move', 'back', 'stream']
"""
```
### task end ###

### task start ###
### code
```python
def square_nums(nums):
  square_nums = list(map(lambda x: x ** 2, nums))
  return square_nums
```

Write the docstring for the above code.

### docstring
```python
"""
Write a function to find squares of individual elements in a list using lambda function.
>>> square_nums([1, 2, 3, 4, 5, 6, 7, 8, 9, 10])
[1, 4, 9, 16, 25, 36, 49, 64, 81, 100]
"""
```
### task end ###
\end{lstlisting}
\end{figure*}

\begin{figure*}[hbt!]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### code
```python
{code}
```

Write the docstring for the above code.

### docstring
```python
{prompt}
```
\end{lstlisting}
\caption{3-shot prompt for getting Reviewer log-likelihoods \citep{coder-reviewer} on HumanEval.}
\label{fig:humaneval_cr_prompt}
\end{figure*}

\begin{figure*}[hbt!]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### code
```python
def count_ways(n):
  A = [0] * (n + 1)
  B = [0] * (n + 1)
  A[0] = 1
  A[1] = 0
  B[0] = 0
  B[1] = 1
  for i in range(2, n+1):
    A[i] = A[i - 2] + 2 * B[i - 1]
    B[i] = A[i - 1] + B[i - 2]
  return A[n]
```

Write the docstring for the above code.

### docstring
```python
"""
Write a function to find the number of ways to fill it with 2 x 1 dominoes for the given 3 x n board.
assert count_ways(2) == 3
"""
```
### task end ###

### task start ###
### code
```python
import re
def find_char_long(text):
  return (re.findall(r"\b\w{4,}\b", text))
```

Write the docstring for the above code.

### docstring
```python
"""
Write a function to find all words which are at least 4 characters long in a string by using regex.
assert find_char_long('Please move back to stream') == ['Please', 'move', 'back', 'stream']
"""
```
### task end ###
\end{lstlisting}
\end{figure*}

\begin{figure*}[hbt!]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### code
```python
def square_nums(nums):
  square_nums = list(map(lambda x: x ** 2, nums))
  return square_nums
```

Write the docstring for the above code.

### docstring
```python
"""
Write a function to find squares of individual elements in a list using lambda function.
assert square_nums([1, 2, 3, 4, 5, 6, 7, 8, 9, 10])==[1, 4, 9, 16, 25, 36, 49, 64, 81, 100]
"""
```
### task end ###

### task start ###
### code
```python
{code}
```

Write the docstring for the above code.

### docstring
```python
{prompt}
```
\end{lstlisting}
\caption{3-shot prompt for getting Reviewer log-likelihoods \citep{coder-reviewer} on MBPP.}
\label{fig:mbpp_cr_prompt}
\end{figure*}

==> sections/sd_prompt.tex <==
\begin{figure*}[t]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### prompt
```python
def count_ways(n):
    """ Write a function to find the number of ways to fill it with 2 x 1 dominoes for the given 3 x n board.
    >>> count_ways(2)
    3
    """
```

### code
```python
def count_ways(n):
    if n == 0:
        return 1
    if n == 1:
        return 1
    if n == 2:
        return 3
    return count_ways(n-1) + count_ways(n-2)
```

### feedback
With the above function, the assertion is `count_ways(2) == 3` and the real execution output is 3. The code passes the assertion.
The code above is incorrect. Please fix it. Make sure the code included in instruction will be executed correctly. Watch out for function/variable names, exception handling, and other errors.

### fixed code
```python
def count_ways(n):
    A = [0] * (n + 1)
    B = [0] * (n + 1)
    A[0] = 1
    A[1] = 0
    B[0] = 0
    B[1] = 1
    for i in range(2, n+1):
        A[i] = A[i - 2] + 2 * B[i - 1]
        B[i] = A[i - 1] + B[i - 2]
    return A[n]
```

### feedback
With the above function, the assertion is `count_ways(2) == 3` and the real execution output is 3. The code passes the assertion.
The code above is correct.
### task end ###
\end{lstlisting}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### prompt
```python
def differ_At_One_Bit_Pos(lhs,rhs):
    """ Write a python function to check whether the two numbers differ at one bit position only or not.
    >>> differ_At_One_Bit_Pos(15,8)
    False
    """
```

### code
```python
def differ_At_One_Bit_Pos(lhs,rhs):
    """ Write a python function to check whether the two numbers differ at one bit position only or not.
    >>> differ_At_One_Bit_Pos(15,8)
    False
    """
    if (lhs - rhs) == 0 or (lhs - rhs) == 1:
        return True
    return False
```

### feedback
With the above function, the assertion is `differ_At_One_Bit_Pos(15,8) == False` and the real execution output is `False`. The code passes the assertion.
The code above is incorrect. Please fix it. Make sure the code included in instruction will be executed correctly. Watch out for function/variable names, exception handling, and other errors.

### fixed code
```python
def differ_At_One_Bit_Pos(a,b):
    """ Write a python function to check whether the two numbers differ at one bit position only or not.
    >>> differ_At_One_Bit_Pos(15,8)
    False
    """
    x = a ^ b
    return x and (not(x & (x - 1)))
```

### feedback
With the above function, the assertion is `differ_At_One_Bit_Pos(15,8) == False` and the real execution output is `False`. The code passes the assertion.
The code above is correct.
### task end ###
\end{lstlisting}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### prompt
```python
def find_char_long(text):
    """ Write a function to find all words which are at least 4 characters long in a string by using regex.
    >>> find_char_long('Please move back to stream')
    ['Please', 'move', 'back', 'stream']
    """
```

### code
```python
def find_char_long(text):
    return (re.findall(r"\b\w{4,}\b", text))
```

### feedback
With the above function, there`s following error:
"""
NameError: name 're' is not defined
"""
The code above is incorrect. Please fix it. Make sure the code included in instruction will be executed correctly. Watch out for function/variable names, exception handling, and other errors.

### fixed code
```python
import re
def find_char_long(text):
    return (re.findall(r"\b\w{4,}\b", text))
```

### feedback
With the above function, the assertion is `find_char_long('Please move back to stream') == ['Please', 'move', 'back', 'stream']` and the real execution output is `['Please', 'move', 'back', 'stream']`. The code passes the assertion.
The code above is correct.
### task end ###
\end{lstlisting}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### prompt
```python
def square_nums(nums):
    """ Write a function to find squares of individual elements in a list using lambda function.
    >>> square_nums([1, 2, 3, 4, 5, 6, 7, 8, 9, 10])
    [1, 4, 9, 16, 25, 36, 49, 64, 81, 100]
    """
```

### code
```python
def square_nums(nums):
    """ Write a function to find squares of individual elements in a list using lambda function.
    >>> square_nums([1, 2, 3, 4, 5, 6, 7, 8, 9, 10])
    [1, 4, 9, 16, 25, 36, 49, 64, 81, 100]
    """
    square_nums = list(map(lambda x: x ** 2, nums))
    return square_nums
```

### feedback
With the above function, the assertion is `square_nums([1, 2, 3, 4, 5, 6, 7, 8, 9, 10]) == [1, 4, 9, 16, 25, 36, 49, 64, 81, 100]` and the real execution output is `[1, 4, 9, 16, 25, 36, 49, 64, 81, 100]`. The code passes the assertion.
The code above is correct.
### task end ###
\end{lstlisting}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### prompt
```python
def find_Rotations(s):
    """ Write a python function to find the minimum number of rotations required to get the same string.
    >>> find_Rotations("aaaa")
    1
    """
```

### code
```python
def find_Rotations(s):
    if len(s) == 1:
        return 1
    elif len(s) == 0:
        return 0
    else:
        l = len(s)
        min = len(s)
        for i, c in enumerate(s):
            if c == s[0]:
                temp = i
                if temp < min:
                    min = temp
        return min
```

### feedback
With the above function, the assertion is `find_Rotations("aaaa") == 1` but the real execution output is `0`.
The code above is incorrect. Please fix it. Make sure the code included in instruction will be executed correctly. Watch out for function/variable names, exception handling, and other errors.

### fixed code
```python
def find_Rotations(s):
    n = len(s)
    for i in range(1, n + 1):
        if s[i:n] + s[0:i] == s:
            return i
    return n
```

### feedback
With the above function, the assertion is `find_Rotations("aaaa") == 1` and the real execution output is `1`. The code passes the assertion.
The code above is correct.
### task end ###
\end{lstlisting}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### prompt
```python
def small_nnum(lst,n):
    """ Write a function to get the n smallest items from a dataset.
    >>> small_nnum([10, 20, 50, 70, 90, 20, 50, 40, 60, 80, 100],2)
    [10, 20]
    """
```

### code
```python
def small_nnum(lst,n):
    """ Write a function to get the n smallest items from a dataset.
    >>> small_nnum([10, 20, 50, 70, 90, 20, 50, 40, 60, 80, 100],2)
    [10, 20]
    """
    lst = sorted(lst)
    lst = lst[:n]
    return lst
```

### feedback
With the above function, the assertion is `small_nnum([10, 20, 50, 70, 90, 20, 50, 40, 60, 80, 100],2) == [10,20]` and the real execution output is `[10, 20]`. The code passes the assertion.
The code above is correct.
### task end ###
\end{lstlisting}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### instruction
{instruction}
```python
{unit_test}
```

### code
```python
{code}
```

###feedback
{feedback}
The code above is 
\end{lstlisting}
\caption{6-shot prompt for self-debugging on HumanEval.}
\label{fig:humaneval_sd_prompt}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### instruction
Write a function to find the number of ways to fill it with 2 x 1 dominoes for the given 3 x n board.
```python
assert count_ways(2) == 3
```

### code
```python
def count_ways(n):
    if n == 0:
        return 1
    if n == 1:
        return 1
    if n == 2:
        return 3
    return count_ways(n-1) + count_ways(n-2)
```

### feedback
With the above function, the assertion is `count_ways(2) == 3` and the real execution output is 3. The code passes the assertion.
The code above is incorrect. Please fix it. Make sure the code included in instruction will be executed correctly. Watch out for function/variable names, exception handling, and other errors.

### fixed code
```python
def count_ways(n):
  A = [0] * (n + 1)
  B = [0] * (n + 1)
  A[0] = 1
  A[1] = 0
  B[0] = 0
  B[1] = 1
  for i in range(2, n+1):
    A[i] = A[i - 2] + 2 * B[i - 1]
    B[i] = A[i - 1] + B[i - 2]
  return A[n]
```

### feedback
With the above function, the assertion is `count_ways(2) == 3` and the real execution output is 3. The code passes the assertion.
The code above is correct.
### task end ###
\end{lstlisting}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### instruction
Write a python function to check whether the two numbers differ at one bit position only or not.
```python
assert differ_At_One_Bit_Pos(15,8) == False
```

### code
```python
def differ_At_One_Bit_Pos(lhs,rhs):
    if (lhs - rhs) == 0 or (lhs - rhs) == 1:
        return True
    return False
```

### feedback
With the above function, the assertion is `differ_At_One_Bit_Pos(15,8) == False` and the real execution output is `False`. The code passes the assertion.
The code above is incorrect. Please fix it. Make sure the code included in instruction will be executed correctly. Watch out for function/variable names, exception handling, and other errors.

### fixed code
```python
def differ_At_One_Bit_Pos(a,b):
  x = a ^ b
  return x and (not(x & (x - 1)))
```

### feedback
With the above function, the assertion is `differ_At_One_Bit_Pos(15,8) == False` and the real execution output is `False`. The code passes the assertion.
The code above is correct.
### task end ###
\end{lstlisting}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[style=markdown]
### task start ###
### instruction
Write a function to find all words which are at least 4 characters long in a string by using regex.
```python
assert find_char_long('Please move back to stream') == ['Please', 'move', 'back', 'stream']
```

### code
```python
def find_char_long(text):
  return (re.findall(r"\b\w{4,}\b", text))
```

### feedback
With the above function, there`s following error:
'''
NameError: name 're' is not defined
'''
The code above is incorrect. Please fix it. Make sure the code included in instruction will be executed correctly. Watch out for function/variable names, exception handling, and other errors.

### fixed code
```python
import re
def find_char_long(text):
  return (re.findall(r"\b\w{4,}\b", text))
```

### feedback
With the above function, the assertion is `find_char_long('Please move back to stream') == ['Please', 'move', 'back', 'stream']` and the real execution output is `['Please', 'move', 'back', 'stream']`. The code passes the assertion.
The code above is correct.
### task end ###
\end{lstlisting}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### instruction
Write a function to find squares of individual elements in a list using lambda function.
```python
assert square_nums([1, 2, 3, 4, 5, 6, 7, 8, 9, 10])==[1, 4, 9, 16, 25, 36, 49, 64, 81, 100]
```

### code
```python
def square_nums(nums):
  square_nums = list(map(lambda x: x ** 2, nums))
  return square_nums
```

### feedback
With the above function, the assertion is `square_nums([1, 2, 3, 4, 5, 6, 7, 8, 9, 10]) == [1, 4, 9, 16, 25, 36, 49, 64, 81, 100]` and the real execution output is `[1, 4, 9, 16, 25, 36, 49, 64, 81, 100]`. The code passes the assertion.
The code above is correct.
### task end ###
\end{lstlisting}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### instruction
Write a python function to find the minimum number of rotations required to get the same string.
```python
assert find_Rotations("aaaa") == 1
```

### code
```python
def find_Rotations(s):
    if len(s) == 1:
        return 1
    elif len(s) == 0:
        return 0
    else:
        l = len(s)
        min = len(s)
        for i, c in enumerate(s):
            if c == s[0]:
                temp = i
                if temp < min:
                    min = temp
        return min
```

### feedback
With the above function, the assertion is `find_Rotations("aaaa") == 1` but the real execution output is `0`.
The code above is incorrect. Please fix it. Make sure the code included in instruction will be executed correctly. Watch out for function/variable names, exception handling, and other errors.

### fixed code
```python
def find_Rotations(s):
  n = len(s)
  for i in range(1, n + 1):
    if s[i:n] + s[0:i] == s:
      return i
  return n
```

### feedback
With the above function, the assertion is `find_Rotations("aaaa") == 1` and the real execution output is `1`. The code passes the assertion.
The code above is correct.
### task end ###
\end{lstlisting}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### instruction
Write a function to get the n smallest items from a dataset.
```python
assert small_nnum([10, 20, 50, 70, 90, 20, 50, 40, 60, 80, 100],2) == [10,20]
```

### code
```python
def small_nnum(lst,n):
  lst = sorted(lst)
  lst = lst[:n]
  return lst
```

### feedback
With the above function, the assertion is `small_nnum([10, 20, 50, 70, 90, 20, 50, 40, 60, 80, 100],2) == [10,20]` and the real execution output is `[10, 20]`. The code passes the assertion.
The code above is correct.
### task end ###
\end{lstlisting}
\end{figure*}

\begin{figure*}[t]
\begin{lstlisting}[style=markdown,escapechar=!]
### task start ###
### instruction
{instruction}
```python
{unit_test}
```

### code
```python
{code}
```

###feedback
{feedback}
The code above is 
\end{lstlisting}
\caption{6-shot prompt for self-debugging on MBPP-S.}
\label{fig:mbpp_sd_prompt}
\end{figure*}

==> sections/sd_results_legacy.tex <==
\begin{table*}[!tb]
\small
\centering
\scalebox{1.1}{
\begin{tabular}{lcccccc@{}}
\toprule
\multirow{2}{*}{Model} & & \multirow{1}{*}{HumanEval(+)} & & & \multirow{1}{*}{MBPP-S(+)} & \\
 &  MBR-Exec & SD-1 & SD-Multi & MBR-Exec & SD-1 & SD-Multi \\ \midrule
\multicolumn{7}{c}{$\sim$7B Scale} \\ \midrule

CL-7B-Instruct& \underline{52.1} (\underline{49.5}) & 52.0 (\underline{49.5}) & \textbf{52.4} (\textbf{50.0}) & 64.0 (57.8) & \underline{65.8} (\underline{59.1}) & \textbf{66.3} (\textbf{60.4}) \\

\rowcolor{softblue}
\quad + Filtering & \underline{74.5} (\underline{70.1}) & 74.4 (\underline{70.1}) & \textbf{76.5} (\textbf{72.3}) & 79.0 (\underline{69.3}) & \underline{79.3} (69.2) & \textbf{81.3} (\textbf{72.1}) \\


DS-6.7B-Instruct& 86.4 (85.5) & \underline{87.0} (\underline{86.0}) & \textbf{87.7} (\textbf{87.0}) & 84.0 (78.6) & \underline{84.6} (\underline{78.8}) & \textbf{84.9} (\textbf{79.3})\\
\rowcolor{softblue}
\quad + Filtering & \textbf{91.6} (\textbf{90.7}) & 91.5 (\underline{90.4}) & \textbf{91.6} (\underline{90.4}) & \underline{89.1} (\underline{82.1}) & 89.0 (81.7) & \textbf{89.9} (\textbf{82.8})  \\

\midrule
\multicolumn{7}{c}{$\sim$13B Scale} \\ \midrule
CL-13B-Instruct& 61.3 (59.6) & \underline{61.7} (\underline{60.1}) & \textbf{62.7} (\textbf{61.4}) & 73.9 (\underline{67.2}) & \textbf{74.4} (67.0) & \textbf{74.4} (\textbf{68.4}) \\
\rowcolor{softblue}
\quad + Filtering & 80.5 (76.1) & \underline{80.9} (\underline{76.5}) & \textbf{81.6} (\textbf{77.6}) & \underline{84.1} (\underline{74.7}) & 83.9 (74.2) & \textbf{84.9} (\textbf{76.2}) \\
\bottomrule
\end{tabular}}%
\caption{Comparison of self-debugging methods with 50 candidates generated by CodeLlama-\{7,13\}B-Instruct with temperature 1.6 and DeepSeekCoder-6.7B-Instruct with temperature 1.2, and debugged over one \citep{chen2024teaching} or multiple candidates using the same LLM. We also provide the upper bound after debugging. Note that results ending with $+$ mean it's evaluated on the plus with extended test cases. Results are averaged across 4 runs.}
\label{tab:sd_results}
\end{table*}
